Elementary totally disconnected, locally compact groups of higher complexity

The article focuses on a class of second countable groups assembled from profinite and discrete by elementary operations. We focus on a rank associated with these groups that measure their complexity, the decomposition rank. A collection of groups acting on $\aleph_0$-regular trees is defined and used for the first construction of a group with decomposition rank $\omega^\omega+1$.

==> drafts.tex <==
\subsection{General theory}

First of all to develop a theory one needs to say what kind of topology will be interesting to make a group into a topological one. We want to have the action on the group itself to be continuous, so asking for the multiplication and inverse being continuous is a reasonable assumption. Another fair hypothesis is that the set with only the identity is closed because otherwise there would be a constant net with only the identity converging to some other element. Assuming both of these one can prove that our space will need to be Hausdorff. With this we get the following definition:

\begin{defi}[Topological group]
Let $(G,*)$ be a group and $\tau$ be a Hausdorff topology on the set $G$. We say $(G,*,\tau)$ is a topological group if the map
$$*(g,h)=gh:G\times G\longrightarrow G \text{ \ and \ } ^{-1}(g)=g^{-1}:G\longrightarrow G$$
is continuous under the topology induced by $\tau$.
\end{defi}
Another equivalent way to define is saying that $\mu (g,h)=gh^{-1}:G\times G\longrightarrow G$ is continuous under the topology $\tau$. To make the notation simpler it will be just said $G$ is a topological group instead of saying $(G,*,\tau)$ is a topological group.\\

\indent Given $G$ a topological group and $a\in G$ we can define the translation maps $\lambda_a(g)=ga:G\longrightarrow G$ and $_a\lambda(g)=ag:G \longrightarrow G$. Given these definitions one can prove the following:


%% Given $V, W\subset G$ and $a\in G$ we will write $aV:={_a\lambda(V)}$, $Va:=\lambda_a(V)$, $V^{-1}:=\{v^{-1}:v\in V\}$, $WV:=\{wv:w\in W, \ v\in V\}=\bigcup_{w\in W} w V$ and $V^n=V^{n-1}V$.

\begin{prop}
Let $G$ be a topological group and $a\in G$. Then:
\begin{itemize}
    \item The maps $_a\lambda:G\longrightarrow G$ and $\lambda_a:G\longrightarrow G$ are homeomorphism of topological spaces;
    \item The map $^{-1}:G\longrightarrow G$ is a homeomorphism of topological spaces.
\end{itemize}
\end{prop}

The continuity of multiplication and inverse makes the topology on a group to be highly symmetric, in the sense that the cosets of a closed/open are also closed/open. One can see that because all cosets of an open subgroup are also open then the complement of an open subgroup is also open, giving the following corollary:

\begin{coro}
Every open subgroup of a topological group is closed.
\end{coro}

When studying topological spaces it is useful to have a notion of when we are sure a subset is closed, open, or compact. The following gives a good idea for it:

\begin{prop}
Let $G$ be a topological group, then the following are true:
\begin{itemize}
    \item If $U$ is an open subset of $G$ and $C$ is any subset, then $UC$ and $CU$ are both open subsets of $G$;
    \item If $K$ is a compact subset of $G$ and $C$ is a closed subset, then $KC$ and $CK$ are both closed subsets of $G$;
    \item If $K_1$ and $K_2$ are compact subsets of $G$ then $K_1K_2$ is a compact subset of $G$.
\end{itemize}
\end{prop}


Just as in any general theory to work with functions between topological groups it is necessary to restrict to the ones that will keep on the property of being a topological group. For this reason, a homomorphism between topological groups is defined as follows:

\begin{defi}[Topological group homomorphism]
Given $G_1$ and $G_2$ topological groups and $$f:G_1\longrightarrow G_2$$ a function. We say $f$ is a topological group homomorphism if it is a homomorphism of groups and it is a continuous function between topological spaces. If $f$ is a group isomorphism and $f^{-1}$ is a continuous function then we say $f$ is an isomorphism of topological groups 
\end{defi}

It is easy to note that given $G$ a topological group and $H\leq G$ then $H$ is a topological group given the subspace topology. One can observe that given an $N\trianglelefteq G$ normal subgroup if we want to make the quotient $\pi:G\rightarrow G/N$ to be continuous one would need the subgroup $N$ to be closed. More than that, if $N$ is not open nor closed then the quotient topology will not even be Hausdorff, hence we get the following result:
\begin{lemma}
Given $G$ a topological group and $N\trianglelefteq G$ a normal subgroup with subspace topology. We have $G/N$ is a topological group with the quotient topology if, and only if, $N$ is a closed subgroup. 
\end{lemma}
An easy example to see what happens when this condition fails is $(\mathbb{Q},+)\trianglelefteq(\mathbb{R},+)$, where $\mathbb{R}$ has the usual topology and $\mathbb{Q}$ has the subspace topology. Because $\mathbb{Q}$ is dense in $\mathbb{R}$ we have that the only closed subsets of $\mathbb{R}/\mathbb{Q}$ are $\emptyset$ and $\mathbb{R}/\mathbb{Q}$.

\begin{prop}
Suppose that $G$ is a compactly generated t.d.l.c.s.c. group, $X$ is a
compact generating set, and $U\in\mathcal{U}(G)$. There is a finite symmetric set $A \subset G$ containing $1$ such that $X \subset AU$ and $UAU=AU$. Further, for any finite symmetric set $A$ containing $1$ with $X \subset AU$ and $UAU=AU$, it is the case that $G = \langle A\rangle U$.
\end{prop}

Given $H$ and $N$ topological groups and $i:H\rightarrow Aut(N)$ a continuous embedding, we can define a semi-direct product of $H$ and $N$ b

Given a short exact sequence $\{1\}\rightarrow N\rightarrow G\rightarrow H\rightarrow \{1\}$ in some cases we can write the group $G$ as a product of the groups $H$ and $K$ in a given way, sometimes with $K$ moving the elements of $H$ around.

\begin{defi}[External semidirect product]\index{external semidirect product}
Let $N$ and $H$ be topological groups and suppose that there is a homomorphism
$$\alpha:h\mapsto \alpha_h\in Aut(N)$$
such that the map $N\times H\rightarrow N:(n,h)\mapsto\alpha_h(n)$ is continuous. Then the external semidirect product of of $N$ and $H$ is the group
$$G=N \rtimes H=\{(n, h) \mid n \in N, h \in H\}$$
equipped with the product $(n_1,h_1)(n_2,h_2)=(n_1\alpha_{h_1}(n_2),h_1h_2)$ and the product topology.
\end{defi}

One can also notice that if a $G$, $N\trianglelefteq G$ and $H\leq G$ are closed subgroup with $G=NH$ and $N\cap H=\{1\}$ then $G$ can be written as $N\rtimes H$ and is said to be the internal direct product of $N$ and $H$.


Ordinal numbers were first defined by Cantor in 1883, in order to work with infinite sequences and classify derived sets, but in the early 1920's von Neumann gave an easier way to define them, which is the one we are using here. The idea is using the empty set, $\emptyset$, as representing $0$ and defining the successor function of a set being $s(S):=S\bigcup \{S\}$, that is, the set that contains all the elements of the original set and with an additional element which is the set itself - note that in ZFC we cannot accept a set which contains itself, hence this function will never be constant.\\ \indent Under this notation we get that $1:=\{\emptyset\}=\{0\}, \ 2:=\{\emptyset,\{\emptyset\}\}=\{0,1\}$ and so on. Allowing arbitrary unions will allow us to define infinite ordinals as well. We denote the first infinite ordinal as $\omega=\{0,1,2,\ldots,n,\ldots\}$. Notice that even with infinite ordinals we can still use the successor operation, for example $s(\omega)=\omega+1=\{0,1,2,\ldots,n,\ldots,\omega\}$.\\
\indent Formally we will define ordinals as follows:

\begin{defi}[Ordinals]\label{defi:ordinals}

We define the ordinal numbers in the following recursive way:
\begin{enumerate}[label=(\roman*)]
    \item[(i)] $0:=\emptyset$ is an ordinal;
    \item[(ii)] Given $\alpha$ an ordinal, $s(\alpha):=\alpha+1$ is also an ordinal;
    \item[(iii)] Given $\{\alpha_i\}_{i\in I}$ a collection of ordinals, $\bigcup_{i\in I}\alpha_i$ is also an ordinal.
\end{enumerate}
\end{defi}
One can see that (i) and (ii) implies that all natural numbers are ordinal numbers. Rule (iii) comes in hand to build infinite ordinals. \\
\indent One important property of ordinal numbers is that given an ordinal number $\alpha$ and defining an order $<$ in it given by $x<y$ if $x\in y$ we have $(\alpha,\in)$ is a well-ordered set. More than that, any well ordered set has an order preserving bijection with an ordinal. With that in mind one can define, alternatively, ordinals as isomorphism classes of well ordered sets.\\
\indent An ordinal $\alpha$ is said to be a successor ordinal if $\alpha=s(\beta)$ for some $\beta$ ordinal. If no such $\beta$ exists then $\alpha$ is said to be a limit ordinal. Examples of limit ordinals are $0, \omega, \omega n$.\\
\indent Given the ordinal numbers, one can also define arithmetic in such a way that restricted to the natural numbers it is the same as the usual one.

\begin{defi}[Ordinal arithmetic]\label{defi:ordinals arithmetic}
Given $\alpha$ and $\beta$ two ordinal, we define the following:
$$\alpha+\beta:=\left\{\begin{array}{ll}
\alpha & \text { if } \beta=0 \\
(\alpha+\gamma)+1 & \text { if } \beta=\gamma+1 \\
\sup _{\gamma<\beta}(\alpha+\gamma) & \text { if } \beta \text { is a limit ordinal}
\end{array}\right.$$
$$\alpha \cdot \beta:=\left\{\begin{array}{ll}
0 & \text { if } \beta=0 \\
(\alpha \cdot \gamma)+\alpha & \text { if } \beta=\gamma+1 \\
\sup _{\gamma<\beta}(\alpha \cdot \gamma) & \text { if } \beta \text { is a limit ordinal}
\end{array}\right.$$
$$\alpha^{\beta}:=\left\{\begin{array}{ll}
1 & \text { if } \beta=0 \\
\left(\alpha^{\beta}\right) \cdot \alpha & \text { if } \beta=\gamma+1 \\
\sup _{\gamma<\beta}\left(\alpha^{\gamma}\right) & \text { if } \beta \text { is a limit ordinal}
\end{array}\right.$$
\end{defi}

Observe that unlike the one for the natural numbers this one is not commutative. One example is the following: $2\omega\neq\omega2$ because $2\omega=\sup_n 2n=\omega$ and $\omega2=\omega+\omega=\sup_n \omega+n=\{0,1,2,\cdots,n,\cdots,\omega,\omega+1,\omega+2,\cdots,\omega+n,\cdots\}$. In a similar way one can see $2^\omega=2+\omega=2\omega=\omega$ but $\omega+2<\omega2<\omega^2$. For the interested reader at \cite{ordinal_text} there is a broader explanation about ordinal arithmetic with a table of sums and multiplications.\\

\begin{defi}[Construction rank]\cite[Definition 3.1]{elementary_first}
For $G\in \mathcal{E}$, define:
\begin{itemize}
    \item $G\in \mathcal{E}_0$ if, and only if, $F$ is either profinite or discrete.
    \item Suppose $\mathcal{E}_\alpha$ is defined. Put $G\in \mathcal{E}_\alpha^{e}$ if and only if there exists $N\trianglelefteq G$ such that $N\in\mathcal{E}_\alpha$ and $G/N\in \mathcal{E}_0$. Put $G\in \mathcal{E}_\alpha^l$ if and only if $G=\cup_{i\in \mathbb{N}}H_i$ where $(H_i)_{i\in \mathbb{N}}$ is an $\subseteq-$increasing sequence of open subgroups of $G$ with $H_i\in \mathcal{E}_\alpha$ for each $i\in \mathbb{N}$. Define $\mathcal{E}_{\alpha+1}:=\mathcal{E}^e_\alpha\cup \mathcal{E}^l_\alpha$.
    \item For $\lambda$ a limit ordinal, $\mathcal{E}_\lambda:=\cup_{\beta<\lambda}\mathcal{E}_\beta$.
\end{itemize}
It is easy to verify that $\mathcal{E}=\cup_{\alpha<\omega_1}\mathcal{E}_\alpha$. We may thus define
$$rk(G):=min\{\alpha|G\in\mathcal{E}_\alpha\}.$$
\end{defi}
By \cite[Proposition 4.20]{elementary_first} we have that if $G\in\mathcal{E}$, then $rk(G)\leqslant 3\xi(G)$ and $\xi(G)\leqslant rk(G)+2$, that is, the difference in both rank is always a finite natural number. For that reason, using the definition of the elementary rank, that has some nicer properties, is similar to using the construction rank.


%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%RESULTS I TOOK OUT THAT ARE REDUNT
%
%
%
%
\begin{lemma}\label{lemma:lower/upper bound}
Suppose that $L$ and $K$ are non-trivial compactly generated elementary groups and $K$ acts on a countable set $X$ with compact open point stabilizers (this action does not need to be faithful). If $U\in \mathcal{U}(L)$ is such that $\overline{\langle\langle U\rangle\rangle_{L}}=L$, then $L\wr_U (K,\ X)$ is elementary with
$$\xi(L)+\alpha\leqslant\xi(L\wr_U(K,\ X))\leqslant\xi(L)+\xi(K)$$
where $\xi(K)=\alpha+2$.
\end{lemma}

\begin{proof}
Set $G:=L\wr_U (K,\ X)$. For the upper bound, Lemma \ref{lemma: rank reduced prod} implies $\xi(\bigoplus_X (L,\ U))=\xi(L)$. Applying Proposition \ref{lemma:short exact sequence elementary rank}, we get that $\xi(G)\leqslant \xi(L)+\xi(K)$, proving our upper bound.\\
\indent For the lower bound, first, we will prove the case $K$ is compact, which implies $\xi(K)\leqslant 2$. In this case, $\bigoplus_X (L,\ U)$ is a normal cocompact subgroup of $G$ hence, by Lemma \ref{lemma:cocompact has same rank as group}, $\xi(\bigoplus_X(L,\ U))=\xi(G)$, verifying the case. From now on, assume $K$ non-compact. \\
\indent Because $K$ is non-compact, there exist $Z\subset X$ an infinite orbit. Fix $Z$ such an orbit. Define $H:=L\wr_U(K,Z)$ and $J:=\bigoplus_Z(L,\ U)$ the subgroups of $L\wr_U(K,\ X)$. We will show that $Res(H)$ contains $J$ and $Res(K)$ as subgroups, making it easier to handle the elementary rank of $H$. The group $H$ is a compactly generated closed subgroup of $G$. Let $O\unlhd H$ be an open normal subgroup. Then $O\cap J$ is an open subgroup of $J$. By the definition of the local direct product (Definition \ref{defi:local direct product}), we can see $J$ as a union of infinite products, all indexed by $Z$. Hence, by the definition of the topology on $J$, $J\cap O$ must contain $U^{Z\setminus I}$ for some finite set $I\subset Z$. The group $K$ acts transitively on $Z$, so $U^Z\leqslant O$. With the assumption $\langle\langle U\rangle\rangle_L=L$, we infer that $\langle \langle U^Z\rangle \rangle_J=J\leqslant O$, hence $J\leqslant Res(H)$. The subgroup $Res(H)$ must also contain the discrete residual of $K$, so
\begin{equation}
    L\wr_U(Res(K),\ X)=J\rtimes Res(K)\leqslant Res(H).
\end{equation}
\indent We now argue by induction on $\alpha$ for the desired inequality.\\
\indent Let $H$ and $J$ be the same as defined above. The base case, $\alpha=0$, follows from the fact $J$ is a closed normal subgroup of $H$ and, by Lemma \ref{lemma:infinite restricted prod rank}, $\xi(J)=\xi(L)$. Suppose the inductive claim holds for all $\beta<\alpha$. Because $K$ is compactly generated, $\xi(K)=\alpha+2$ for some $\alpha$ ordinal. Set $R:=Res(K)$ and let $R=\bigcup_{j\in \mathbb{N}}E_j$, with $E_j$ an increasing sequence of compactly generated open subgroups of $R$. Each $E_j$ is compactly generated. Since $\xi(R)<\xi(K)$, for every $j\in\mathbb{N}$ $\xi(E_j)=\beta_j+2$, for some $\beta_j<\alpha$.\\
\indent For each $j\in \mathbb{N}$, the group $\bigoplus_Z(L,\ U)\rtimes E_j=L\wr_U(E_j,Z)$ has, by the inductive hypothesis, $\xi(L)+\beta_j\leqslant\xi(L\wr_U(E_j,Z))$.\\
\indent The group $L\wr_U(R,Z)$ is an increasing union of the open subgroups $L\wr_U(E_j,Z)$, so
$$\xi(L)+\sup_{j\in\mathbb{N}}\beta_j\leqslant \xi(L\wr_U(R,Z)).$$
Hence, by $(1)$, we get $\xi(L)+\sup_{j\in\mathbb{N}}(\beta_j)\leqslant \xi(L\wr_U(R,Z))\leqslant \xi(Res(H))$. We thus deduce that $\xi(L)+\sup_{j\in\mathbb{N}}(\beta_j)+1\leqslant \xi(H)$.\\
\indent Observe that $\sup_{j\in\mathbb{N}}(\beta_j)+1\leqslant\xi(R)\leqslant\sup_{j\in\mathbb{N}}(\beta_j)+2$, where the exact value corresponds to whether the supremum is a limit ordinal or a successor ordinal. On the other hand, $\xi(K)=\xi(R)+1=\alpha+2$, so $\alpha\leqslant\sup_{j\in\mathbb{N}}(\beta_j)+1$ in either case for $\xi(R)$. With this we get that $\xi(L)+\alpha\leqslant\xi(H)\leqslant\xi(G)$, completing the induction.
\end{proof}

%%Unlike Lemma \ref{lemma: bad bound}, Lemma \ref{lemma:lower/upper bound} lets us quite close to the upper bound on the wreath product rank.

\begin{prop}\label{prop:making group with compact open that becomes entire group get higher rank}
Suppose that $(G,\ X)$ is a compactly generated non-trivial transitive elementary permutation group. If $U\in \mathcal{U}(G)$ is such that $\overline{\langle\langle U\rangle\rangle_{G}}=G$, then $E_X(G,\ U)$ has rank
$$\xi(E_X(G,\ U))=\omega^{\beta+1}+2$$
where $\beta$ is the leading exponent in the Cantor normal form of $\xi(G)$. If $G$ is also topologically perfect, then $P_X(G,\ U)$ is the monolith and has rank $\omega^{\beta+1}+1$.
\end{prop}

\begin{proof}
Let $\alpha$ be such that $\xi(G)=\alpha+2$. Then the leading exponent of $\xi(G)$ and of $\alpha$ are the same. Let $\beta$ be the leading exponent. The sum of $n$ copies of $\xi(G)$ and $m$ copies of $\alpha$ is thus always bounded below by $\omega^{\beta}(m+n)$.  On the other hand, the sum of any number of finite copies of $\xi(G)$ is always bounded by $\omega^{\beta+1}$. With this in mind and applying Lemma \ref{lemma:lower/upper bound} we see that for all $n\in\mathbb{N}$ we have
\begin{equation}\label{equation:2}
    \omega^\beta n \leqslant \xi(G_n)< \omega^{\beta+1}
\end{equation}
, where $G_n$ is defined as the iterated wreath product of $G$ $n$ times, as in Definition \ref{defi:wr product}.\\
\indent By colouring the tree $\vec{T_{\chi}}$, fixing $v\in V\vec{T_{\chi}}$ and defining $T_0$, $T_R$ as in Lemma \ref{lemma:Gn 101}, we get an embedding of the iterated wreath product $G_n$ as a closed subgroup of $E_X(G,\ U)_{(T_R)}$, for each $n\geqslant 1$.\\
\indent Let $L_n$, $W_{(T_0)}$ and $H_n$ be the subgroups as defined in the proof of Proposition \ref{prop:grp is elementary}. As seen in Proposition \ref{prop:grp is elementary}, the subgroups $H_n$ are open in $P_X(G,\ U)$, and for $n\in\mathbb{N}$ the subgroup $L_n W_{(T_0)}$ is compact and normal in $H_n$, with $H_n/L_nW_{(T_0)}\cong G_n$. We thus deduce that $H_n$ is an open elementary subgroup of $P_X(G,\ U)$. Furthermore, Lemma \ref{lemma:lower/upper bound} and (\ref{equation:2}) ensure
\begin{equation}\label{eq:3}
    \omega^\beta n\leqslant \xi(H_n)< \omega^{\beta+1}.
\end{equation}
\indent The collection $\{H_n\}_{n\in\mathbb{N}}$ is directed. So $\bigcup_{n\in\mathbb{N}}H_n$ is an open elementary subgroup of $P_X(G,\ U)$. Applying Lemma \ref{lemma:Gn 101} it follows that
$$\bigcup_{n\in\mathbb{N}}H_n=E_X(G,\ U)_{(T_R)}W_{(T_0)}.$$
Moreover, following the fact that the rank of a group is the supremum of the rank of all open subgroups, equation (\ref{eq:3}) gives us that $\xi(E_X(G,\ U)_{(T_R)}W_{(T_0)})=\omega^{\beta+1}+1$. Fixing $t$ a translation toward $\delta$, the family $(t^n E_X(G,\ U)_{(T_R)}W_{(T_0)}t^{-n})_{n\geqslant 0}$ is directed. In view of Lemma \ref{lemma:Gn 101} we get that
$$\bigcup_{n\geqslant 0}t^n E_X(G,\ U)_{(T_R)}W_{(T_0)}t^{-n}=P_X(G,\ U)$$,
and in view of Proposition \ref{prop:grp is elementary}, $\xi(P_X(G,\ U))=\omega^{\beta+1}+1$.\\
\indent The discrete residual of $E_X(G,\ U)$ is contained in $P_X(G,\ U)$, that is $\xi(Res(E_X(G,\ U)))\leqslant \xi(P_X(G,\ U))$. Thus, $\xi(E_X(G,\ U))=\xi(Res(E_X(G,\ U)))+1\leqslant \xi(P_X(G,\ U))+1$, and we deduce that $$\omega^{\beta+1}+1\leqslant\xi(E_X(G,\ U))\leqslant \omega^{\beta+1}+2.$$
Non-trivial compactly generated groups cannot have an elementary rank of the form $\lambda+1$, with $\lambda$ a limit ordinal, thus $\xi(E_X(G,\ U))=\omega^{\beta+1}+2$.\\
\indent The final claim is immediate from Proposition \ref{prop: monolith tree}.
\end{proof}

==> residual_order_first_draft.tex <==

Given $G$ a t.d.l.c.s.c. group and $S\subset Aut(G)$ is a subset (no topology is given to $Aut(G)$), we define the discrete residue of $S$ in relation to $G$ as:
$$Res_G(S):=\bigcap\{O;O\text{ is an open subgroup of } G \text{, and }\phi(O)=O \text{ for every }\phi\in S\}.$$
In a similar way, if $\psi:H\rightarrow Aut(G)$ is a group homomorphism, we can define $Res_G(H)$ under this automorphism. One example that we will use a lot is one can define the discrete residue of subgroups of $G$ under $inn:G\rightarrow Aut(G)$. Notice that $Res_G(G)=Res(G)$, where $Res(G)$ is defined as in Definition \ref{defi:discrete residue}.\\
\indent If $H,N$ are subgroups of $G$ and $H$ normalizes $N$ then $Res_N(H)$ can be defined in a similar way, as $H$ can be seen as a subgroup of $Aut(N)$.

\begin{defi}[Residual order]
Let $G$ be a topological group. We define the discrete residue order on $\mathcal{K}(G)$ given by $H_1\preccurlyeq H_2$ if $H_1<Res_G(H_2)$ and $Res_G(H_1)< Res_G(H_2)$, or $H_1=H_2$. If $H_1\preccurlyeq H_2$ and $H_1\neq H_2$ we will denote it as $H_1\prec H_2$.
\end{defi}

\begin{lemma}\label{lemma:partial order} 
Given $G$ a topological group then the residual order on $\mathcal{K}(G)$ is a partial order.
\end{lemma}

\begin{proof}
The reflexivity follows from definition. Assume $H_1\preccurlyeq H_2$ and $H_2\preccurlyeq H_3$. By assumption, if $O\leqslant G$ is an open subgroup such that for all $h_3\in H_3$ we have $h_3O=Oh_3$, then $H_2\leqslant O$. Hence if for all $h_3\in H_3$, $h_3O=Oh_3$ then $h_2O=Oh_2$ for every $h_2\in H_2$, that is, $H_1\leqslant O$. Then $H_1<Res_G(H_3)$, that is, $H_1\preccurlyeq H_3$. Hence the order is transitive.\\
\indent Let $K_1,K_2\in\mathcal{K}(G)$ such that $K_1\preccurlyeq K_2\preccurlyeq K_1$. If $K_1\neq K_2$ then $Res_G(K_1)<Res_G(K_2)<Res_G(K_1)$, a contradiction. Hence $K_1=K_2$, that is, the order is antisymmetric.
\end{proof}

Lemma \ref{lemma:partial order} shows us that there are no cycles when looking at the residual order. This allow us to define a rank in relation to this order in a t.d.l.c.s.c. group.

\begin{defi}[Residual height and rank]\label{defi:residual height/rank}
Let $G$ be a topological group and $H\in \mathcal{K}(G)$. We define the residual height of $H$ in relation to $G$, $\textphnc{y}_G(H)$, as follows
$$\textphnc{y}_G(H)=\left\{ \begin{array}{ll}
    1 & \mbox{if }Res_G(H)=\{1\}, \\
   \sup_{H'\prec H} \textphnc{y}_G(H)+1 & \mbox{otherwise.}
\end{array}  \right.$$
and the residual rank of $G$ as
$$\textphnc{f}(G)=\left\{ \begin{array}{ll}
    1 & \mbox{if }G=\{1\}, \\
   \sup_{H\in \mathcal{K}(G)}\textphnc{y}_G(H)+1. & \mbox{otherwise.}
\end{array}  \right.$$
\indent If for every $H\in \mathcal{K}(G)$, $\textphnc{y}(H)<\omega_1$ we say that the residual rank is well defined in $G$.
\end{defi}

Note that if $L\leqslant G$ is a compactly generated, because $Res_L(L)\leqslant Res_G(L)$, $\textphnc{y}_L(L)\leqslant \textphnc{y}_G(L)$. Also, a consequence of the elementary rank being well defined for elementary groups is that the residual height and rank is always well defined for elementary groups. We will now show useful properties of the residual rank.

\begin{lemma}
Let $G$ be a t.d.l.c.s.c. group. For every $H\in \mathcal{K}(G)$ we have that $\textphnc{y}_G(H)=\textphnc{y}_G(\overline{H})$.
\end{lemma}

\begin{proof}
Follows from the fact $Res_G(H)=Res_G(\overline{H})$.
\end{proof}

\begin{prop}\label{prop:rank 2 is the same in both ranks}
Let $G$ be a t.d.l.c. group. Then $G$ is elementary with $\xi(G)=2$ if, and only if, $\textphnc{f}(G)=2$.
\end{prop}

\begin{proof}
Assume $\xi(G)=2$. Let $H\in \mathcal{K}(G)$ non-trivial and $U$ be a compact open subgroup of $G$. The subgroup $O=\langle U,H\rangle\leqslant G$ is a compactly generated open subgroup. Because $O$ is non-trivial then $\xi(O)=2$ and because $O$ is compactly generated then $Res(O)=\{1\}$. Because $Res_G(H)\leqslant Res(O)$ then $Res_G(H)=\{1\}$ and $\textphnc{y}(H)=1$. Then $\textphnc{f}(G)=2$.\\
\indent If $\textphnc{f}(G)=2$ then for every $H\in\mathcal{K}(G)$, $\textphnc{y}(H)=1$. This implies that for every $O\leqslant G$ compactly generated open subgroup of $G$, $Res(O)=\{1\}$, hence $\xi(G)=2$.
\end{proof}

\begin{theorem}[\cite{residual_theorem_colin}, Theorem  G]\label{thrm:colin result for res commuting}
Let $G$ be a t.d.l.c. group and $H\leqslant Aut(G)$ a compactly generated subgroup. Then $Res_{Res_G(H)}(H)=Res_G(H)$.
\end{theorem}

For the next result notice that given $G$ a group and $H\in\mathcal{K}(G)$ we have that $Res_G(H)=Res_G(H\backslash H\cap Z(G))$, because if $h\in H\cap Z(G)$ then $hO=Oh$ for every open subgroup of $O\leqslant G$. Also, if $H,N_1,N_2$ are subgroups of $G$ such that $H$ normalizes $N_1, N_2$ and $N_1\geqslant N_2$, then $Res_G(H)\geqslant Res_{N_1}(H)\geqslant Res_{N_2}(H)$.

\begin{prop}\label{prop:easier residual height}
Let $G$ be a t.d.l.c. group with well defined residual height. Then:
\begin{itemize}
    \item If $O\leqslant G$ is open and $H\leqslant O$ is compactly generated then $\textphnc{y}_O(H)=\textphnc{y}_G(H)$
    \item If $H\leqslant Res(G)$ is compactly generated then $\textphnc{y}_{Res(G)}(H)=\textphnc{y}_G(H)$.
\end{itemize}
\end{prop}

\begin{proof}
Let $O\leqslant G$ an open subgroup and $H\leqslant O$ a compactly generated subgroup. Notice that $V\leqslant G$ an open subgroup is such that $hVh^{-1}=V$ for every $h\in H$ if, and only if, $h(V\cap O)h^{-1}=V\cap O$ for every $h\in H$. Hence $Res_O(H)=Res_G(H)$ and the result follows.\\
\indent Assume now that $H\leqslant Res(G)$. Notice that $Res_G(H)\geqslant Res_{Res(G)}(H) \geqslant Res_{Res_G(H)}(H)$. By Theorem \ref{thrm:colin result for res commuting} the result follows.
\end{proof}

With these results we can prove the similarities between the residual rank and the elementary rank:

\begin{prop}\label{coro:simplified residual rank on compactly generated}
Let $G$ be a compactly generated t.d.l.c. group. If $Res(G)$ has a well defined residual height then $\textphnc{f}(G)=\textphnc{y}(G)+1=\textphnc{f}(Res(G))+1$.
\end{prop}

\begin{proof}
To prove $\textphnc{f}(G)=\textphnc{y}(G)+1$ notice that if $H_1\prec H_2$ then $H_1\leqslant Res_G(H_2)\leqslant Res(G)$, hence $H_1\prec G$, that is, the height of $G$ is maximal on $G$.\\
\indent By definition and the fact $\textphnc{f}(G)=\textphnc{y}(G)+1$ it follows that $\textphnc{f}(G)=(\sup_{H\prec G}\textphnc{y}(H)+1)+1$. Because $H\prec G$ implies $H\leqslant Res(G)$, Proposition \ref{prop:easier residual height} implies $\textphnc{f}(G)=\textphnc{f}(Res(G))+1$.
\end{proof}

\begin{prop}\label{coro:simplified residual rank general}
Let $G$ be a t.d.l.c. group and $\{O_n\}_{n\in\mathbb{N}}$ an increasing collection of compactly generated subgroups of $G$ with well defined residual height such that $G=\cup_{n\in\mathbb{N}}O_n$.  Then $\textphnc{f}(G)=\sup_{n\in\mathbb{N}}(\textphnc{f}(Res(O_n)))+1$.
\end{prop}

\begin{proof}
Let $H$ a compactly generated subgroup of $G$ and $H=\langle K\rangle$, with $K$ compact. Because $\{O_n\}$ is a covering of $K$ then there is $N\in\mathbb{N}$ such that for every $n\geqslant N$ then $K\subset O_n$, hence $H\leqslant O_n$. By Proposition \ref{prop:easier residual height} it follows that $\textphnc{y}_{O_n}(H)=\textphnc{y}_{G}(H)$. By Corollary \ref{coro:simplified residual rank on compactly generated} it follows that $\sup_{H\in\mathcal{K}(G)}\textphnc{y}_G(H)=\sup_{n\in\mathbb{N}}\textphnc{y}_G(O_n)$ and hence $\textphnc{f}(G)=\sup_{n\in\mathbb{N}}(\textphnc{y}(O_n))+1=\sup_{n\in\mathbb{N}}(\textphnc{f}(Res(O_n)))+1$.
\end{proof}


\begin{theorem}\label{thrm:for elementary groups ranks are the same}
If $G$ is an elementary group then $\xi(G)=\textphnc{f}(G)$.
\end{theorem}

\begin{proof}
If $\xi(G)=1$ or $\textphnc{f}(G)=1$ then $G=\{1\}$ and the result follows. By Proposition \ref{prop:rank 2 is the same in both ranks} the result is also true when $\xi(G)=2$.\\
\indent Assume that for every $\beta<\alpha$ if $G$ is elementary with $\xi(G)=\beta+1$ then $\textphnc{f}(G)=\beta+1$. Let $G$ be a elementary group such that $\xi(G)=\alpha+1$. We will now break the induction hypothesis in the case $G$ is compactly generated and when it is not.\\
\indent Assume $G$ is compactly generated. Then $\xi(G)=\xi(Res(G))+1$ and, by the induction hypothesis, the residual rank of $Res(G)$ is well defined and $\xi(Res(G))=\textphnc{f}(Res(G))$. By Corollary \ref{coro:simplified residual rank on compactly generated} it follows that $\textphnc{f}(G)=\textphnc{f}(Res(G))+1$ hence the results follows for one direction.\\
\indent On the other hand, let $G$ not compactly generated. Let $\{O_n\}_{n\in\mathbb{N}}$ be an increasing collection of open compactly generated subgroups such that $G=\cup_{n\in\mathbb{N}}O_n$. Then, for every $n\in\mathbb{N}$, $\xi(O_n)\leqslant \alpha+1$. If there exist $N\in\mathbb{N}$ such that for every $n\geq N$, $\xi(O_n)=\alpha+1$, the argument for compactly generated groups of rank $\alpha+1$ implies that $\xi(O_n)=\textphnc{f}(O_n)$. If for every $n\in\mathbb{N}$, $\xi(O_n)<\alpha+1$, because they are all compactly generated, the induction hypothesis implies $O_n$ has a well defined residual rank and $\textphnc{f}(O_n)=\xi(O_n)$. In either case, Corollary \ref{coro:simplified residual rank general} implies $\textphnc{f}(G)=\sup_{n\in\mathbb{N}}(\textphnc{f}(Res(O_n)))+1=\sup_{n\in\mathbb{N}}(\xi(Res(O_n)))+1=\xi(G)=\alpha+1$.
\end{proof}

\begin{theorem}[\cite{residual_theorem_colin}, Theorem  B]\label{thrm:colin theorem G}
Let $G$ be a t.d.l.c. group and let $H$ be a compactly generated subgroup of $G$. Then there is an open subgroup $E$ of $G$ with the following properties:
\begin{enumerate}
    \item  $E = H Res_G(H)U$, where $U$ is a compact open subgroup of $G$;
    \item $E$ is compactly generated;
    \item $Res_G(H) = Res(E)$, so in particular, $Res_G(H)$ is normal in $E$.
\end{enumerate}
\end{theorem}

\begin{coro}
Let $G$ be an elementary group. If $H\in \mathcal{K}(G)$ then there exists $E$ an open compactly generated subgroup of $G$ such that $\textphnc{f}(E)=\textphnc{y}_G(E)+1=\textphnc{y}_G(H)+1$.
\end{coro}

\begin{proof}
Let $E$ be an open, compactly generated subgroup such that $Res_G(H)=Res(E)$, as given in Theorem \ref{thrm:colin theorem G}. Because $E$ is open then, by Proposition \ref{prop:easier residual height}, $\textphnc{y}_G(E)=\textphnc{y}_E(E)\geqslant \textphnc{y}_G(H)=\textphnc{y}_E(H)$ but, because $Res_G(H)=Res(E)$, we get $\textphnc{y}_E(H)= \textphnc{y}_E(E)$. Hence the result follows.
\end{proof}

\begin{lemma}\label{lemma:residual rank and semidirect product}
Let $G$ be a t.d.l.c. group. If $G=N\rtimes K$ and $H$ is a compactly generated closed subgroup of $K$ such that $N\rtimes H$ is compactly generated, then $Res_G(N\rtimes H)\geqslant Res_K(H)$.
\end{lemma}
 
\begin{proof}
Let $O\leqslant_o G$ an open subgroup such that for every $g\in N\rtimes H$ we have $gO=Og$. Notice that under this assumption, $O\cap K$ is open in $K$ and for every $h\in H$ we have $h(O\cap K)=(O\cap K)h$, hence the result follows. 
\end{proof}

\begin{lemma}\label{lemma:finite products and residual height}
Let $G_1,G_2,\ldots,G_n$ be t.l.c. groups with well defined residual height. Then
$$\textphnc{f}\left(\prod_{i=1}^n G_i\right)\geqslant \sup_{1\leqslant i\leqslant n}\left(\textphnc{y}_{G_i}(G_i)\right)+1$$
with equality if, and only if, for every $1\leqslant i \leqslant n$ and every $K_i\in\mathcal{K}(G_i)\backslash\{1\}$ we have that $Res_{G_i}(K_i)\cap K_i<K_i$.
\end{lemma}

\begin{proof}
The proof will be given for $n=2$ and it follows easily by induction for all other cases. \\
\indent Let $K\in \mathcal{K}(G_1\times G_2)$. Then $K=K_1\times K_2$, for $K_i$ a closed compactly generated subgroup of $G_i$, $i=1,2$. Notice that $Res_G(K)=Res_{G_1}(K_1)\times Res_{G_2}(K_2)$, hence if $K'\prec K$ then $K_1'\prec K_1$ or $K_2'\prec K_2$. Hence the inequality follows.\\
\indent If for $i=1,2$ and every $K_i\in \mathcal{K}(G_i)$ we have that $Res_{G_i}(K_i)\cap K_i<K_i$ then if $K,K'\in\mathcal{K}(G)$ are such that $K'\prec K$ the conditions imply that $K_1'\prec K_1$ and $K_2'\prec K_2$. Hence the equality holds.\\
\indent Assume there exists $K_1\in\mathcal{K}(G_1)\backslash\{1\}$ such that $K_1\leqslant Res_{G_1}(K_1)$. Given $\alpha<\textphnc{y}_{G_2}(G_2)$ let $\{K_{(\alpha,\beta+1)}\}_{\beta<\alpha}\subset \mathcal{K}(G_2)$ be a collection such that $\textphnc{y}_{G_2}(K_{(\alpha,\beta+1)})=\beta+1$ and for $\beta_1<\beta_2$ we have that $K_{(\alpha,\beta_1+1)}\prec K_{(\alpha,\beta_2+1)}$. Then 
$$\textphnc{y}_{G_1\times G_2}\left(K_1,K_{(\alpha,\beta+1)}\right)\geqslant \beta+1+\textphnc{y}_{G_1}(K_1)$$
which implies
$$\textphnc{f}(G_1\times G_2)\geqslant \textphnc{f}(G_2)-1+\textphnc{y}_{G_1}(K_1)+1.$$
\end{proof}



\begin{coro}\label{coro:residual height and restricted product}
Given $\{G_n\}_{n\in\mathbb{N}}$ a collection of t.d.l.c groups with well defined residual height and $U_n\in \mathcal{U}(G_n)$, for each $n\in\mathbb{N}$. Then
$$\textphnc{f}\left(\oplus_{n\in\mathbb{N}}(G_n,U_n)\right)\geqslant\sup_{n\in \mathbb{N}}\left(\textphnc{y}_{G_n}(G_n)\right)+1$$
with equality if, and only if, for every $n\in\mathbb{N}$ and every $K_n\in \mathcal{K}(G_n)\backslash\{1\}$ we have that $Res_{G_n}\cap K_n<K_n$.
\end{coro}

\begin{proof}
Follows from Lemma \ref{lemma:finite products and residual height}, Corollary \ref{coro:simplified residual rank general} and the fact that the restricted product (Definition \ref{defi:local direct product}) can be seen as the union of the subgroups $S_i$, as defined earlier, the result follows.
\end{proof}

Given $G$ a group with well defined residual height, we say that $G$ is well behaved under the discrete residue order if for every $K\in\mathcal{K}(G)$ we have $Res_G(K)\cap K<K$.\\
\indent Notice that elementary groups always satisfy the condition for the equality.

\begin{lemma}\label{lemma:decreasing residual height}
Let $G$ be a t.d.l.c.s.c. group well behaved under the discrete residue. Given $H\leqslant G$ a subgroup (not necessarily closed) then $H$ is well behaved under the discrete residue. More than that, if $K\in\mathcal{K}(H)$ then $\textphnc{y}_H(K)\leqslant \textphnc{y}_G(K)$.
\end{lemma}

\begin{proof}
Fix $K\in\mathcal{K}(H)\subset \mathcal{K}(G)$. Given $O\leqslant G$ such that $kO=Ok$ for every $k\in K$, notice that $O\cap H$ is such that $k(O\cap H)=(O\cap H) k$ for every $k\in K$,  hence
$$ Res_H(K)   \leqslant  O\cap H  \leqslant  O $$
   $$   Res_H(K)   \leqslant  \bigcap_{\substack{O\leqslant_o G \\ kO=Ok,  \forall k\in K}} O\cap H  \leqslant  \bigcap_{\substack{O\leqslant_o G \\ kO=Ok,  \forall k\in K}}O  =  Res_G(K). $$
Taking intersection under $K$ we get, by the hypothesis, that
$$Res_H(K)\cap K\leqslant Res_G(K)\cap K<K$$
hence $H$ is also well behaved under the discrete residue.\\
\indent To show $\textphnc{y}_H(K)\leqslant \textphnc{y}_G(K)$, let $K_1\in\mathcal{K}(H)$ be such that $K_1\prec K$ in relation to $H$. We need to prove that this implies $K_1\prec K$ in relation to $G$.
%Let $K_1,K_2\in\mathcal{K}(H)$ be such that $K_1\prec K_2$ in relation to $H$. We will prove that this implies $K_1\prec K_2$ in relation to $G$, therefore $\textphnc{y}_H(K)\leqslant \textphnc{y}_G(K)$.\\
%\indent By the assumption we have that $K_1<Res_H(K_2)$ and $Res_H(K_1)<Res_H(K_2)$. It follows from the definition of the discrete residue in relation to a group that $K_1<Res_H(K_2)\leqslant Res_G(K_2)$. Because $G$ is elementary it is also true that $Res_G(K_1)< K_1\geqslant Res_G(K_2)<K_2$
%Let $O\leqslant G$ an open subgroup such that for every $k\in K$ we have $kO=Ok$. It is easy to see that $k(O\cap K)=(O\cap K)k$, hence $Res_H(K)\leqslant Res_G(K)\cap K$.
\end{proof}

\subsection{Building elementary groups with given rank}

\begin{defi}
Let $G$ be a compactly generated group with well defined residual rank. We say that a collection $\{G_{\beta+1}\}_{\beta<\alpha}$ of closed compactly generated subgroups of $G$ witness that the rank of $G$ is greater than $\alpha+2$ if for every $\beta<\alpha$, $\textphnc{y}_G(G_{\beta+1})=\beta+1$ and if $\beta<\beta'$ then  $G_{\beta+1}<Res_G(G_{\beta'+1})$, $Res_G(G_{\beta+1})<Res_G(G_{\beta'+1})$. If $\textphnc{f}(G)=\alpha+2$ we say that this chain witness the rank of $G$.
\end{defi}

Notice that it might be possible for a group to have rank $\omega+2$ but have no collection of groups that witness the rank of $G$, an example of that would be a compactly generated group $G$ can only have a chain of finitely many groups less than it, but these chains can be as big as one wants.\\
\indent A group $G$ with rank $\omega+2$ that has a collection of groups witnessing the rank will have a collection of compactly generated subgroups that can be ordered in the following way:

$$\begin{tikzcd}
G_1 & G_2 \arrow[l] & G_3 \arrow[l] & \ldots \arrow[l] & G_{\omega+1} \arrow[l]
\end{tikzcd}$$

\noindent and a group $G$ with rank $\omega+2$ that has no collection of groups witnessing the rank might have a collection of compactly generated subgroups that can be ordered in the following way:

$$\begin{tikzcd}
          &                     & G_{\omega+1} \arrow[lld] \arrow[ld] \arrow[d] \arrow[rd] \arrow[rrd] &                     &        \\
G_1^{(1)} & G_2^{(2)} \arrow[d] & G_3^{(3)} \arrow[d]                                                  & G_4^{(4)} \arrow[d] & \ldots \\
          & G_1^{(2)}           & G_2^{(3)} \arrow[d]                                                  & G_3^{(4)} \arrow[d] &        \\
          &                     & G_1^{(3)}                                                            & G_2^{(4)} \arrow[d] &        \\
          &                     &                                                                      & G_1^{(4)}           &       
\end{tikzcd}$$

\begin{theorem}\label{thrm:making big ranks better with residue order}
Suppose $L$ and $K$ are non-trivial compactly generated groups, $K$ is well behaved under the discrete residue order, and $K$ acts on a countable set $X$ with compact open point stabilizers (the action does not need to be faithful). If $U\in\mathcal{U}(L)$ is such that $\langle\langle U\rangle \rangle_L=L$ and there exists $\{K_{\alpha+1}\}_{\alpha<\textphnc{f}(K)-1}$ a chain witnessing the rank of $K$ such that $K_1$ has one infinite orbit $Y_1\subset X$ then
$$\textphnc{f}(L\wr_U(K,X))\geqslant \textphnc{y}_L(L)+\textphnc{y}_K(K)+1=\textphnc{f}(L)-1+\textphnc{f}(K)+1.$$
\end{theorem}

\begin{proof}
Let $\{K_{\alpha+1}\}_{\alpha<\textphnc{f}(K)-1}$ be a chain witnessing the rank of $K$ and $Y_1\subset X$ an infinite orbit of $K_1$. For each $\alpha<\textphnc{f}(K)-1$ define the subsets $Y_{\alpha+1}:=K_{\alpha+1}Y_{1}$, and the subgroups $G_{\alpha+1}:=L\wr_U(H_{\alpha+1},Y_{\alpha+1})$, $J_{\alpha+1}:=\oplus_{y\in Y_{\alpha+1}}(L,U)$, and $G:=L\wr_U(K,X)$. Notice that because the action of $K_{\alpha+1}$ in $Y_{\alpha+1}$ are transitive, the groups $G_{\alpha+1}$ are compactly generated.\\
\indent Claim 1: $J_1< Res_G(G_1)$ and if $\alpha<\beta$ then $G_{\alpha+1}<Res_G(G_{\beta+1})$.\\
\indent Let $O\leqslant G$ be an open subgroup such that for every $g\in G_{\alpha+1}$ we have $gO=Og$. Then $O$ contains an open subgroup of $J_{\alpha+1}$ and, for the reason that $J_{\alpha+1}\leqslant G_{\alpha+1}$, we have $O\cap J_{\alpha+1}$ is normal in $J_{\alpha+1}$. Since $J_{\alpha+1}$ is an union of an increasing family of infinite products all indexed by $Y_{\alpha+1}$, as in Definition \ref{defi:local direct product}, then $O$ contains $U^{Y_{\alpha+1}\backslash I}$, for some finite set $I\subset Y_{\alpha+1}$. The group $K_{\alpha+1}$ acts transitively on $Y_{\alpha+1}$, so $U^{Y_{\alpha+1}}\leqslant O$. Because $O\cap J_{\alpha+1}$ is normal on $J_{\alpha+1}$ and $\langle\langle U\rangle \rangle_L=L$ we get that $\oplus_{y\in Y_{\alpha+1}}(L,U)\leqslant O$, hence $\oplus_{y\in Y_{\alpha+1}}(L,U)\leqslant Res_G(G_{\alpha+1})$. The subgroup $Res_G(G_{\alpha+1})$ must also contain $Res_K(K_{\alpha+1})$, by Lemma \ref{lemma:residual rank and semidirect product}, so
$$L\wr_U(Res_K(K_{\alpha+1}),Y_{\alpha+1})=J_{\alpha+1}\rtimes Res_K(K_{\alpha+1})\leqslant Res_G(G_{\alpha+1})$$
proving the claim.\\
\indent Claim 2: $\textphnc{y}_L(L)+1\leqslant\textphnc{y}_G(G_1)$.\\
\indent Corollary \ref{coro:residual height and restricted product} implies that $\textphnc{f}(J_1)=\textphnc{y}_{J_1}(J_1)\geqslant \textphnc{y}_L(L)+1$. For the reason that $K$ is well behaved under the discrete residue order, $Res_{G}(J_1)<J_1\leqslant Res_G(G_1)$ hence, together with Claim $1$ and the observation after Definition \ref{defi:residual height/rank} we get that $\textphnc{y}_G(G_1)\geqslant \textphnc{y}_G(J_1)+1 \geqslant\textphnc{y}_L(L)+1$.\\
\indent Claim 3: If $\alpha<\beta$, $Res_G(G_{\alpha+1})<Res_G(G_{\beta+1})$.\\
\indent AAA\\
\indent To finish the proof, the claims and Definition \ref{defi:residual height/rank} implies that $\textphnc{y}_G(G_1)\geqslant \textphnc{y}_L(L)+1$ and $\textphnc{y}_G(G)\geqslant \textphnc{y}_G(G_1)-1+\textphnc{y}_K(K)$, hence
%$$\textphnc{f}(G)=\textphnc{y}_G(G)+1\geqslant \textphnc{y}_L(L)+\textphnc{y}_K(K)+1.$$
\end{proof}



\begin{coro}
If $L$ and $K$ are groups satisfying the conditions from Theorem \ref{thrm:making big ranks better with residue order} and $\textphnc{f}(K)>\omega$ then the condition of $K_1$ having an infinite orbit $Y_1\subset X$ is not necessary.
\end{coro}

\begin{proof}
Let $\{K_{\alpha+1}\}_{\alpha<\textphnc{f}(K)-1}$ be a collection of compactly generated subgroups of $K$ that witness the rank of $K$. Notice that even though $K_1$ might not have an infinite orbit in $X$, $K_2$ will have one infinite orbit, say $Y_2$. With the notation and proof from Theorem \ref{thrm:making big ranks better with residue order} we get that
$$$$
\end{proof}

\begin{coro}\label{coro:still have chain witnessing the rank}
If $L$ and $K$ are elementary groups satisfying the conditions from Theorem \ref{thrm:making big ranks better with residue order}, or from Corollary \ref{thrm:making big ranks better with residue order}, and $L$ has a chain witnessing its rank then $L\wr_U(K,X)$ has a chain witnessing that the rank is $\textphnc{y}_L(L)+\textphnc{y}_K(K)+1$. If $L=K$ then the group $E_X(L,U)$ has a chain witnessing that its rank.
\end{coro}

\begin{proof}
Denote $G:=L\wr_U(K,X)$ and let $\{L_{\alpha+1}\}_{\alpha<\textphnc{f}(L)-1}$, $\{K_{\beta+1}\}_{\beta<\textphnc{f}(K)-1}$ be chains witnessing the rank of $L$ and $K$, respectively. Given $y\in Y_1$ define $L^{y_K}_{\alpha+1}\leqslant \oplus_{x\in X_K}(L,U)$ the subgroup that is $L_{\alpha+1}$ in the $y_K$ coordinate and the trivial group for $x\neq y_K$. For $\beta<\textphnc{y}_K(K)$ define $X_{\beta+1}=K_{\beta+1} Y_K$. Then, for $\gamma<\textphnc{y}_L(L)+\textphnc{y}_K(K)$ we define $G_{\gamma+1}$ as follows:
$$G_{\gamma+1}:=\left\{\begin{array}{ll}
    L^{y_L}_{\gamma+1} & \mbox{if }\gamma<\textphnc{f}(L)-1   \\
    \oplus_{x\in X_{\beta+1}}(L,U)\rtimes K_{\beta+1} & \mbox{if } \gamma=\textphnc{f}(L)-1+\beta. 
\end{array}
\right.$$
then Theorem \ref{thrm:making big ranks better with residue order} implies that given $\gamma<\gamma'$ then $G_{\gamma+1}<Res_G(G_{\gamma'+1})$, $Res_G(G_{\gamma+1})<Res_G(G_{\gamma'+1})$. The condition that $\textphnc{y}_G(G_{\gamma+1})\geqslant \gamma+1$ follows from the construction.\\
\indent For $E_X(L,U)$ and let $L_n< E_X(L,U)$ be the iteration of the wreath product as defined after \ref{defi:wr product}. By Theorem \ref{thrm:making big ranks better with residue order} we have that $L_1<L_2<\ldots<L_n<\ldots$ and by the argument above $L_n$ has a chain witnessing that its rank is greater or equal than $\textphnc{y}_L(L).n+2$ and the chain of $L_i$ is contained in $L_j$, for $i<j$. Let $\{G_{\gamma+1}\}_{\gamma<\textphnc{y}_L(L).\omega}$ be the upper bound of these chains, then it is a chain of $E_X(L,U)$ witnessing that the rank is greater or equal than $\textphnc{y}_L(L).\omega+1$. Proposition \ref{prop:making group with compact open that becomes entire group get higher rank} implies that $L_n< Res(E_X(L,U))$, for all $n\in\mathbb{N}$, hence we can increase the size of the chain witnessing the rank of $E_X(L,U)$ by $1$, that is, there is a chain of $E_X(L,U)$ witnessing that its rank is $\omega+2$. 
\end{proof} 

\begin{coro}\label{coro:condition for the rank to be additive}
If $L$ and $K$ are elementary groups satisfying the conditions from Theorem \ref{thrm:making big ranks better with residue order} and $\xi(K)\geqslant \omega+2$ then 
$$\xi(L\wr_U(K,X))=\xi(L)+\xi(K).$$
\end{coro}

\begin{proof}
By Theorem \ref{thrm:for elementary groups ranks are the same} it follows that $\xi(L\wr_U(K,X))=\textphnc{y}(L\wr_U(K,X))$ and the inequality from Theorem \ref{thrm:making big ranks better with residue order} become
$$\xi(L\wr_U(K,X))\geqslant \xi(L)-1+\xi(K)$$
but, because $\xi(K)>\omega$ and the fact $\xi(L\wr_U(K,X))\leqslant \xi(L)+\xi(K)$ (Lemma \ref{lemma:lower/upper bound}) it follows that
$$\xi(L\wr_U(K,X))= \xi(L)+\xi(K).$$
\end{proof}

\begin{coro}\label{coro:adding 1 to the rank}
If $L$ satisfies the conditions from Theorem \ref{thrm:making big ranks better with residue order}, and $(K,X)$ is a permutation group satisfying the conditions from Theorem \ref{thrm:result for higher rank by wesolek}. Then 
$$\textphnc{f}(L\wr_U(K,X))=\textphnc{f}(L)+1.$$
\end{coro}

\begin{proof}
By the proof of Theorem \ref{thrm:making big ranks better with residue order} we that 
$$Res(L\wr_U(K,X))\geqslant \oplus_{x\in X}(L,U)\rtimes Res_K(K)=\oplus_{x\in X}(L,U)$$
and, because $\oplus_{x\in X}(L,U)$ is an open, normal subgroup of $L\wr_U(K,X)$ then
$$Res(L\wr_U(K,X))\leqslant \oplus_{x\in X}(L,U)$$
That is, $Res(L\wr_U(K,X))=\oplus_{x\in X}(L,U)$. Hence by Corollary \ref{coro:residual height and restricted product} we have \break $\textphnc{y}_{L\wr_U(K,X)}(L\wr_U(K,X))=\textphnc{y}_L(L)+1$.
\end{proof}



\begin{prop}\label{prop:making other properties work addition on rank}
Let $L, K$ be non-trivial compactly generated groups and $X_L, X_K$ countable sets. If $L$ acts on $X_L$ and $K$ acts on $X_K$ with compact open point stabilizers (the action does not need to be faithful), there exists $U_L\in\mathcal{U}(L)$, $U_K\in \mathcal{U}(K)$ such that $\langle\langle U_L\rangle \rangle_L=L$, $\langle\langle U_K\rangle \rangle_K=K$ then $G:=K\wr_{U_L}(L,X_K)$ acts on $X:=X_L\times X_K$ with compact open point stabilizers and $U:=\prod_{x\in X_K}U_L\rtimes U_K$ is a compact open subgroup of $G$ such that $\langle\langle U\rangle\rangle_G=G$.
\end{prop}

\begin{proof}
Because $G$ is a wreath product we define its action on $X$ as the imprimitive action, hence it has compact open point stabilizers. It is easy to see that $\langle \langle U\rangle \rangle_G=G$. 
\end{proof}

With these results and Theorem \ref{thrm:result for higher rank by wesolek} we have all that is necessary to build a group with a given elementary rank below $\omega^\omega+1$. For the sake o f concreteness we will simplify a notation to build them and give an example of how it can be done.\\

\begin{notation}[Iterated wreath product]
Let $(G,X)$, $(G',X')$ and $(G'',X'')$ be permutation t.d.l.c.s.c. groups and $U\in\mathcal{U}(G), \ U'\in\mathcal{U}(G'), \ U''\in\mathcal{U}(G'')$ fixed open, compact subgroups. We denote by 
$$G\wr_{U}G'\wr_{U'}G'':=G\wr_{U}(G'\wr_{U'}(G'',X''),(X'\times X''))$$
where the action of the groups is given by the imprimitive action as defined in \ref{defi:wr product}.\\
\indent For $(G,X)$ a permutation group and $U\in\mathcal{U}(G)$ we will denote
$$G_1:=G, \ U_1:= U$$
and for $n>1$
$$G_n:=G\wr_{U}(G_{n-1},X^{n-1}), \ U_{n}:=\prod_{x\in X^{n-1}}U\rtimes U_{n-1}.$$
\end{notation}

Now, for the construction, let $\alpha< \omega^\omega+1$ be a non limit ordinal. Using the Cantor normal form we can write it as
$$\alpha=\sum_{i=1}^n \omega^i a_i+(a_0+1)$$
where $a_i\in \mathbb{N}$. Pick a group $G$ satisfying the conditions from Theorem \ref{thrm:result for higher rank by wesolek} and build the permutation groups $(F_n(G),X_n)$ and its subgroups $U_n(G)$ as in the theorem. If $a_0>0$ then we build the compactly generated topologically perfect groups
$$(F_n(G))_{a_n}\wr_{(U_n(G))_{a_n}}(F_{n-1}(G))_{a_{n-1}}\wr_{(U_{n-1}(G))_{a_{n-1}}}\ldots\wr_{(U_{1}(G))_{a_1}} (F_0(G))_{a_0}$$
and for $a=0$ the group
$$Res((F_n(G))_{a_n}\wr_{(U_n(G))_{a_n}}(F_{n-1}(G))_{a_{n-1}}\wr_{(U_{n-1}(G))_{a_{n-1}}}\ldots\wr_{(U_{1}(G))_{a_1}} (F_0(G))_{1})$$
which by definition of the elementary rank, Corollaries \ref{coro:condition for the rank to be additive} and \ref{coro:adding 1 to the rank} imply that these groups have rank $\alpha$.\\
\indent One can also build a group with rank $\omega^\omega+1$ as follows:
$$\bigoplus_{n\in\mathbb{N}}(F_n(G),U_n(G)).$$
The rank of this group follows from Proposition \ref{prop:product same rank}, the definition of local direct product (Definition \ref{defi:local direct product}) and the definition of elementary rank (Definition \ref{defi:elementary rank}).
